WordCraft: An Environment for Benchmarking Commonsense Agents

The ability to quickly solve a wide range of real-world tasks requires a commonsense understanding of the world. Yet, how to best extract such knowledge from natural language corpora and integrate it with reinforcement learning (RL) agents remains an open challenge. This is partly due to the lack of lightweight simulation environments that sufficiently reflect the semantics of the real world and provide knowledge sources grounded with respect to observations in an RL environment. To better enable research on agents making use of commonsense knowledge, we propose WordCraft, an RL environment based on Little Alchemy 2. This lightweight environment is fast to run and built upon entities and relations inspired by real-world semantics. We evaluate several representation learning methods on this new benchmark and propose a new method for integrating knowledge graphs with an RL agent.

==> core/1_introduction_alternative.tex <==
\section{Introduction}
\label{sec:intro}
Recent progress in Reinforcement Learning (RL) has been impressive \citep{silver2016mastering, vinyals2019alphastar, DBLP:journals/corr/abs-1912-06680}, but it has mostly been fueled by \emph{tabula-rasa} learning. 
For example, while Go is an extremely difficult game to master, its rules and thus environment dynamics are simple, not heavily relying on knowledge about concepts that can be encountered in the real world.
Focusing on tabula-rasa learning confines state-of-the-art approaches to simulation environments that can be solved without requiring transfer of commonsense, world or domain-knowledge. However, many real-world applications (e.g., personal assistants and household robots) require agents that can learn fast and generalize well to unseen situations, something that is likely not possible without commonsense and general knowledge about the world. 

Humans communicate much of their knowledge through written language, for example on Wikipedia.
Outside of RL, learning to represent and utilize such knowledge have improved considerably over the last years.
For example, a common approach is to pre-train neural language models and fine-tuning them on downstream tasks~\citep{DBLP:conf/naacl/DevlinCLT19,DBLP:journals/corr/abs-1910-10683}.
Recent works highlight that such pre-trained models capture several aspects of common-sense~\citep{DBLP:journals/corr/abs-1910-01157} and relational knowledge~\citep{DBLP:conf/emnlp/PetroniRRLBWM19}, in addition to linguistic knowledge~\citep{DBLP:conf/acl/JawaharSS19,DBLP:conf/naacl/HewittM19,DBLP:conf/nips/ReifYWVCPK19}.
Another approach is to represent commonsense knowledge explicitly in Knowledge Graphs (KGs), such as ATOMIC~\citep{DBLP:conf/aaai/SapBABLRRSC19} and ConceptNet~\citep{speer2017conceptnet}.
However, the question how to best utilize knowledge (either in texts or KGs) for downstream RL environments has not received the same level of attention, partly due scarce simulation environments that directly benefit from transeferring such knowledge.

To address the shortage of fast simulation environments that put emphasis on knowledge transfer, we present AlchemyCraft, a small environment that is easy to run, composed of over N hundred entities, M relations between them ground wrt external knowledge sources (recipe list, ConceptNet, GloVe embeddings etc.).

% thus, there is a disconnect wrt progress of deep RL in these simulation environments and their applicability to more real-world tasks

% to overcome these issues, we present AlchemyCraft: small environment that is easy to run, composed of over N hundred entities, M relations between them ground wrt external knowledge sources (recipe list, ConceptNet, GloVe embeddings etc.), and bc 

% in AlchemyCraft, the agent is tasked to TODO

% in addition, we develop a knowledge graph conditioned policy learner
% we show that by learning to utilize ground-truth knowledge graphs, this approach can zero-shot TODO
% furthermore, by building upon recent neural link prediction work our agents are able to utilize partial knowledge graphs, inferring missing relations and employing this knowledge to learn faster and generalize to unseen concepts

% By isolating the problem of knowledge transfer and planning from high-dimensional obsrevation spaces and TODO, we believe AlchemyCraft will spur reesarch in BLAH


% TIM'S OUTLINE

% existing progress in RL impressive, but generally done via tabula-rasa learning 
% existing environments often do not require transfer of commonsense, world or domain knowledge (e.g. Go); or they are costly to run and are hard to ground to external knowledge sources (e.g. SC2)

% thus, there is a disconnect wrt progress of deep RL in these simulation environments and their applicability to more real-world tasks

% to overcome these issues, we present AlchemyCraft: small environment that is easy to run, composed of over N hundred entities, M relations between them ground wrt external knowledge sources (recipe list, ConceptNet, GloVe embeddings etc.), and bc 

% in AlchemyCraft, the agent is tasked to TODO

% in addition, we develop a knowledge graph conditioned policy learner
% we show that by learning to utilize ground-truth knowledge graphs, this approach can zero-shot TODO
% furthermore, by building upon recent neural link prediction work our agents are able to utilize partial knowledge graphs, inferring missing relations and employing this knowledge to learn faster and generalize to unseen concepts

% By isolating the problem of knowledge transfer and planning from high-dimensional obsrevation spaces and TODO, we believe AlchemyCraft will spur reesarch in BLAH

